High Performance and Portable Convolution Operators for ARM-based Multicore Processors

The considerable impact of Convolutional Neural Networks on many Artificial Intelligence tasks has led to the development of various high performance algorithms for the convolution operator present in this type of networks. One of these approaches leverages the \imcol transform followed by a general matrix multiplication (GEMM) in order to take advantage of the highly optimized realizations of the GEMM kernel in many linear algebra libraries. The main problems of this approach are 1) the large memory workspace required to host the intermediate matrices generated by the IM2COL transform; and 2) the time to perform the IM2COL transform, which is not negligible for complex neural networks. This paper presents a portable high performance convolution algorithm based on the BLIS realization of the GEMM kernel that avoids the use of the intermediate memory by taking advantage of the BLIS structure. In addition, the proposed algorithm eliminates the cost of the explicit IM2COL transform, while maintaining the portability and performance of the underlying realization of GEMM in BLIS.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> s6n-future.tex <==
\paragraph{Future work.}
This work yields a considerable amount of open research and development lines, listed in the following:
\begin{enumerate}
    \item Full integration of the optimized convolution algorithm within the BLIS library.
    \item Implementation of other similar transforms (\textsc{col2im}) with transposed \gemm kernels needed in
          the back-propagation stage for DNN training.
\item Evaluation of the approach on alternative low-power processors: ARM Cortex-A7, Cortex-A15, Cortex-A53, NVIDIA Denver,\ldots.
       This only requires specific architecture-specific micro-kernels for these other architectures. 
\item Development of the \convgemm scheme for inference with fixed point and integer models/arithmetic. 
      This only requires architecture-specific micro-kernel.
\item Development of the \convgemm scheme for the RISC-V processor.
      This architecture may not support cache coherence in hardware, but integrate a scratchpad cache. This implies
      that the \gemm code must explicitly move data in and out of the cache. This is similar to previous
      work on adapting BLIS for Texas Instruments digital signal processors (DSPs); see \url{https://arxiv.org/abs/1908.11263}.
\item Comparison with other portable libraries for convolution: NNPACK and QNNPACK.
%\begin{quote} 
%From: \url{https://research.fb.com/wp-content/uploads/2018/12/Machine-Learning-at-Facebook-Understanding-Inference-at-the-Edge.pdf}\\
%NNPACK (Neural Networks PACKage) per- forms computations in 32-bit floating-point precision and NCHW layout, and targets high-intensity convo- lutional neural networks, which use convolutional oper- ators with large kernels, such as 3x3 or 5x5. NNPACK implements asymptotically fast convolution algorithms, based on either Winograd transform or Fast Fourier transform, which employ algorithmic optimization to lower computational complexity of convolutions with large kernels by several times. With algorithmic advan- tage and low-level microarchitecture-specific optimiza- tions, NNPACK often delivers higher performance for direct convolution implementation.\\
%NNPACK, “Acceleration package for neural networks on multi-core cpus.”
%https://github.com/Maratyszcza/NNPACK
%QNNPACK (Quantized NNPACK) on the other hand performs computations in 8-bit fixed-point pre- cision and NHWC layout. It is designed to augment NNPACK for low-intensity convolutional networks, e.g. neural networks with large share of 1x1, grouped, depth- wise, or dilated convolutions. These types of convolu- tions do not benefit from fast convolution algorithms, thus QNNPACK provides a highly efficient implementa- tion of direct convolution algorithm. Implementation in QNNPACK eliminates the overhead of im2col transfor- mation and other memory layout transformations typ- ical for matrix-matrix multiplication libraries. Over a variety of smartphones, QNNPACK outperforms state- of-the-art implementations by approximately an aver- age of two times.\\
%M. Dukhan, Y. Wu, and H. Lu, “QNNPACK: open source library for optimized mobile deep learning.” https://code.fb.com/ml- applications/qnnpack
%
%\end{quote} 
\item Extension for \convgemm based on Strassen multiplication; see \url{http://jianyuhuang.com/papers/sc16.pdf}.
\item Extension of \convgemm based on Winograd filters.
\item Extension for convolution on ARM asymmetric systems-on-chip (e.g., ARM big.LITTLE).
\item Leverage that, for inference, the weights do not change. Therefore, pack the matrix containing
      that information once and re-use multiple times, as proposed in~\cite{Dukh19}. 
\end{enumerate}

